Benchmarking Foundation Models for Zero-Shot Biometric Tasks

The advent of foundation models, particularly Vision-Language Models (VLMs) and Multi-modal Large Language Models (MLLMs), has redefined the frontiers of artificial intelligence, enabling remarkable generalization across diverse tasks with minimal or no supervision. Yet, their potential in biometric recognition and analysis remains relatively underexplored. In this work, we introduce a comprehensive benchmark that evaluates the zero-shot and few-shot performance of state-of-the-art publicly available VLMs and MLLMs across six biometric tasks spanning the face and iris modalities: face verification, soft biometric attribute prediction (gender and race), iris recognition, presentation attack detection (PAD), and face manipulation detection (morphs and deepfakes). A total of 41 VLMs were used in this evaluation. Experiments show that embeddings from these foundation models can be used for diverse biometric tasks with varying degrees of success. For example, in the case of face verification, a True Match Rate (TMR) of 96.77 percent was obtained at a False Match Rate (FMR) of 1 percent on the Labeled Face in the Wild (LFW) dataset, without any fine-tuning. In the case of iris recognition, the TMR at 1 percent FMR on the IITD-R-Full dataset was 97.55 percent without any fine-tuning. Further, we show that applying a simple classifier head to these embeddings can help perform DeepFake detection for faces, Presentation Attack Detection (PAD) for irides, and extract soft biometric attributes like gender and ethnicity from faces with reasonably high accuracy. This work reiterates the potential of pretrained models in achieving the long-term vision of Artificial General Intelligence.

==> bios/bio_redwan.tex <==
Redwan Sony (Graduate Student Member, IEEE) received the B.Sc. degree in computer science and engineering from the Islamic University of Technology (IUT), Bangladesh, in 2016, and the M.Sc. degree in computer science and engineering from Michigan State University, in 2023, where he is currently pursuing the Ph.D. degree. He is currently a Research Assistant with the iPRoBe Laboratory, Michigan State University, under the supervision of Prof. Arun Ross. From 2017 to 2021, he was a Lecturer with the Department of Computer Science and Engineering, IUT. His research interests include facial and forensic biometrics, model visualization, and the explainability of deep learning models.

==> bios/bio_rossarun.tex <==
Arun Ross (Senior Member, IEEE) received the B.E. degree (Hons.) in computer science from BITS Pilani, India, and the M.S. and Ph.D. degrees in computer science and engineering from Michigan State University, USA. He is currently the Martin J. Vanderploeg Endowed Professor with Michigan State University and the Site Director of the NSF Center for Identification Technology Research. He has co-authored the textbook, Introduction to Biometrics and the monograph, Handbook of Multibiometrics. He was a recipient of the NSF CAREER Award and was designated as a Kavli Fellow by the U.S. National Academy of Sciences, in 2006. He received the J. K. Aggarwal Prize, in 2014, and the Young Biometrics Investigator Award, in 2013, from the International Association of Pattern Recognition. He has advocated for the responsible use of biometrics in multiple forums including the NATO Advanced Research Workshop on Identity and Security in Switzerland, in 2018. He testified as an Expert Panelist in an event organized by the United Nations Counter-Terrorism Committee at the UN Headquarters, in 2013. In June 2022, he testified at the U.S. House Science, Space, and Technology Committee on the topic of Biometrics and Personal Privacy.

==> sections/biographies.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/img_redwan.png}}]{Redwan Sony}\input{bios/bio_redwan}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/img_redwan.png}}]{Parisa Farmanifard }\input{bios/bio_redwan}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/img_redwan.png}}]{ Alzwairy}\input{bios/bio_redwan}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/img_redwan.png}}]{ Nitish Shukla}\input{bios/bio_redwan}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/img_redwan.png}}]{ Arun  Ross}\input{bios/bio_rossarun}
\end{IEEEbiography}


==> tables/ethnicity_classification_one_shot.tex <==
\begin{table*}[ht]
\caption{Benchmarking ethnicity classification accuracy (\%) on the VMER~\cite{Greco_MVA2020_VMER} dataset using features extracted by various VLMs. One-shot classification results are averaged over 5-fold cross-validation. A shallow classifier is trained on the extracted features to evaluate performance. Variance is ignored for brevity.}
\centering
\begin{tabular}{l|c|c|c|c|c}
\hline

Model & \textbf{KNN} & \textbf{LDA} & \textbf{Logistic } & \textbf{Ridge} & \textbf{SVM}\\
 &\cite{cover1967nearest} & \cite{fisher1936use_lda} & \textbf{Regression}~\cite{fisher1936use_lda} &\textbf{Regression}~\cite{hoerl1970ridge} & \cite{cortes1995svm} 
\\\hline
\hline
Salesforce\_blip-image-captioning-base & 89.16 & 94.82 & 94.08 & 94.30 & 92.82 \\
Salesforce\_blip-image-captioning-large & 91.48 & 95.76 & 94.84 & 95.48 & 93.80 \\\hline
Salesforce\_blip2-flan-t5-xl & 98.88 & 97.60 & 97.92 & 97.64 & 97.78 \\
Salesforce\_blip2-flan-t5-xl-coco & 97.98 & 97.20 & 97.32 & 97.18 & 97.56 \\
Salesforce\_blip2-flan-t5-xxl & 98.90 & 97.64 & 97.92 & 97.62 & 97.76 \\
Salesforce\_blip2-opt-2.7b & 98.90 & 97.60 & 97.92 & 97.62 & 97.80 \\
Salesforce\_blip2-opt-6.7b & 98.88 & 97.62 & 97.92 & 97.62 & 97.76 \\\hline
facebook\_dino-vitb16 & 78.80 & 85.84 & 84.40 & 85.76 & 82.12 \\
facebook\_dinov2-base & 85.30 & 91.56 & 89.88 & 91.28 & 89.80 \\
facebook\_dinov2-giant & 86.34 & 92.00 & 93.00 & 92.44 & 92.32 \\
facebook\_dinov2-large & 85.92 & 92.66 & 92.26 & 92.36 & 91.68 \\
facebook\_dinov2-small & 82.02 & 88.42 & 86.52 & 87.84 & 83.68 \\\hline
facebook\_sam-vit-base & 64.44 & 74.18 & 76.00 & 76.00 & 76.00 \\
facebook\_sam-vit-huge & 64.74 & 75.82 & 76.00 & 76.00 & 76.00 \\
facebook\_sam-vit-large & 64.06 & 74.56 & 76.00 & 76.00 & 76.00 \\\hline
google\_vit-base-patch16-224 & 89.46 & 93.04 & 90.98 & 92.80 & 91.12 \\
google\_vit-base-patch16-384 & 90.76 & 93.56 & 91.94 & 93.48 & 91.52 \\
google\_vit-base-patch32-384 & 89.34 & 92.06 & 89.14 & 91.94 & 89.54 \\
google\_vit-huge-patch14-224-in21k & 88.72 & 90.64 & 89.42 & 90.28 & 89.68 \\
google\_vit-hybrid-base-bit-384 & 90.48 & 93.86 & 92.70 & 93.36 & 92.36 \\
google\_vit-large-patch16-224 & 89.82 & 92.90 & 92.72 & 92.82 & 92.32 \\
google\_vit-large-patch16-384 & 90.52 & 93.72 & 93.44 & 93.56 & 93.08 \\
google\_vit-large-patch32-384 & 88.06 & 92.50 & 90.34 & 92.26 & 91.24 \\\hline
hf-hub:laion\_CLIP-ViT-B-32-laion2B-s34B-b79K & 97.48 & 95.48 & 95.08 & 94.66 & 95.94 \\
hf-hub:laion\_CLIP-ViT-H-14-laion2B-s32B-b79K & 98.98 & 97.24 & 96.32 & 96.00 & 97.26 \\
hf-hub:laion\_CLIP-ViT-g-14-laion2B-s12B-b42K & 98.86 & 97.28 & 96.18 & 95.98 & 97.06 \\
hg-hub:laion\_CLIP-ViT-H-14-laion5B-s13B-b90k & 98.98 & 97.24 & 96.32 & 96.00 & 97.26 \\\hline
kakaobrain\_align-base & 95.84 & 96.30 & 96.32 & 96.18 & 96.12 \\\hline
llava-hf\_llava-1.5-7b-hf & 99.38 & 97.74 & 98.26 & 97.70 & 98.56 \\
llava-hf\_llava-v1.6-mistral-7b-hf & 89.50 & 52.94 & 95.96 & 95.78 & 96.46 \\\hline
openai\_clip-vit-base-patch16 & 98.60 & 97.08 & 97.26 & 96.94 & 97.86 \\
openai\_clip-vit-base-patch32 & 97.78 & 96.70 & 97.14 & 96.34 & 96.98 \\
openai\_clip-vit-large-patch14 & 99.28 & 97.68 & 97.98 & 97.54 & 98.30 \\
openai\_clip-vit-large-patch14-336 & 99.38 & 97.70 & 98.22 & 97.70 & 98.56 \\
\hline
\end{tabular}
\label{tab:ethnicity_classification_table}

\end{table*}
